Understanding Dementia Speech Alignment with Diffusion-Based Image Generation

Text-to-image models generate highly realistic images based on natural language descriptions and millions of users use them to create and share images online. While it is expected that such models can align input text and generated image in the same latent space little has been done to understand whether this alignment is possible between pathological speech and generated images. In this work, we examine the ability of such models to align dementia-related speech information with the generated images and develop methods to explain this alignment. Surprisingly, we found that dementia detection is possible from generated images alone achieving 75% accuracy on the ADReSS dataset. We then leverage explainability methods to show which parts of the language contribute to the detection.

==> tables/ECS_score.tex <==
\begin{table}[h]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{l|cc}
        \hline
        \textbf{Group} & \multicolumn{2}{c}{\textbf{Extraneous Content Score (ECS)}} \\
        & \textbf{Original} & \textbf{No Discourse} \\
        \hline
        AD & 0.6736 & 0.6633 \\
        CC & 0.7505 & 0.7407 \\
        \hline
    \end{tabular}
    \caption{Comparison of Extraneous Content Score (ECS) for AD and CC groups before and after removal of discourse tokens.}
    \label{tab:voluntary_addition}
\end{table}


==> tables/fidelity_metrics.tex <==
\begin{table*}[h]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{l|c|cc|cc}
        \hline
        \textbf{Group} & \textbf{IU Present} & \multicolumn{2}{c|}{\textbf{CLIP}} & \multicolumn{2}{c}{\textbf{TIFA}} \\
        &  & \textbf{Original} & \textbf{No Discourse} & \textbf{Original} & \textbf{No Discourse} \\
        \hline
        AD & 7.2083 & 0.1575 & 0.1634 & 0.2786 & 0.2877 \\
        CC & 12.625 & 0.1502 & 0.1566 & 0.2322 & 0.2093 \\
        \hline
    \end{tabular}
    \caption{Comparison of IU present, CLIP, and TIFA scores for AD and CC groups.}
    \label{tab:iu_clip_tifa}
\end{table*}


==> tables/image_quality_metrics.tex <==
\begin{table*}[h]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{l|cc|cc|cc}
        \hline
        \textbf{Model} & \multicolumn{2}{c|}{\textbf{IS}} & \multicolumn{2}{c|}{\textbf{FID}} & \multicolumn{2}{c}{\textbf{LPIPS}} \\
        & \textbf{Original} & \textbf{No Discourse} & \textbf{Original} & \textbf{No Discourse} & \textbf{Original} & \textbf{No Discourse} \\
        \hline
        AD & 3.1626 $\pm$ 0.4352 & 3.6194 $\pm$ 0.6615 & 425.2882 & 433.0645 & 0.7145 & 0.7167 \\
        CC & 3.0784 $\pm$ 0.3795 & 3.0841 $\pm$ 0.3105 & 435.9554 & 411.1374 & 0.7207 & 0.7318 \\
        \hline
    \end{tabular}
    \caption{Comparison of IS, FID, and LPIPS scores for AD and CC groups with and without discourse tokens in the input prompt.}
    \label{tab:is_fid_lpips}
\end{table*}

